Optimal Algorithms for Continuous Non-monotone Submodular and DR-Submodular Maximization

In this paper we study the fundamental problems of maximizing a continuous non-monotone submodular function over the hypercube, both with and without coordinate-wise concavity. This family of optimization problems has several applications in machine learning, economics, and communication systems. Our main result is the first $\frac{1}{2}$-approximation algorithm for continuous submodular function maximization; this approximation factor of $\frac{1}{2}$ is the best possible for algorithms that only query the objective function at polynomially many points. For the special case of DR-submodular maximization, i.e. when the submodular functions is also coordinate wise concave along all coordinates, we provide a different $\frac{1}{2}$-approximation algorithm that runs in quasilinear time. Both of these results improve upon prior work [Bian et al, 2017, Soma and Yoshida, 2017]. Our first algorithm uses novel ideas such as reducing the guaranteed approximation problem to analyzing a zero-sum game for each coordinate, and incorporates the geometry of this zero-sum game to fix the value at this coordinate. Our second algorithm exploits coordinate-wise concavity to identify a monotone equilibrium condition sufficient for getting the required approximation guarantee, and hunts for the equilibrium point using binary search. We further run experiments to verify the performance of our proposed algorithms in related machine learning applications.

==> results.tex <==
\section{Main Theoretical Results}


%\paragraph{Tight approximation for continuous submodular
%  maximization.} Our first main result is a %tight
%$\frac{1}{2}$-approximation algorithm (up to additive $\delta>0$
%error) for maximizing a continuous submodular function $\F$,
%a.k.a. \texttt{weak DR-SM}, which is information-theoretically 
%%tight under standard complexity
%theoretic assumptions
%optimal~\citep{feige2011maximizing}. 
%This result assumes that $\F$ is coordinate-wise Lipschitz
%continuous.\footnote{Such an assumption is necessary, since otherwise the
%  single-dimensional problem amounts to optimizing an arbitrary function and
%  is hence intractable. Prior work,
%  e.g.~\cite{bian2017guaranteed} and \cite{bian2017continuous},
%  implicitly requires such an assumption to perform single-dimensional optimization.}

%\begin{equation*}
%\forall i\in[n],\forall \xv_{-i}:~~x^*_i=\underset{z\in[0,1]}{\argmax}~\F(z,\xv_{-i}),
%\end{equation*}
%\paragraph{Quasilinear time algorithm for \texttt{\textbf{strong DR-SM}} maximization.} Our second result is a fast binary search algorithm, achieving the tight $\frac{1}{2}$-approximation factor (up to additive error $\delta$) in quasi-linear time in $n$, but  only for the special case of a DR-submodular function $\F$, i.e. \texttt{strong DR-SM}. This algorithm leverages the coordinate-wise concavity to identify a coordinate-wise \emph{monotone equilibrium condition}. In each iteration, it hunts for an equilibrium point by using binary search. Satisfying the equilibrium at each iteration then guarantees the desired approximation factor.  To handle the error of binary search in continuous space for each coordinate, we impose a mild technical assumption and assume $\F$ is coordinate-wise Lipschitz continuous.



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

